New Job, New Gender? Measuring the Social Bias in Image Generation Models

Image generation models can generate or edit images from a given text. Recent advancements in image generation technology, exemplified by DALL-E and Midjourney, have been groundbreaking. These advanced models, despite their impressive capabilities, are often trained on massive Internet datasets, making them susceptible to generating content that perpetuates social stereotypes and biases, which can lead to severe consequences. Prior research on assessing bias within image generation models suffers from several shortcomings, including limited accuracy, reliance on extensive human labor, and lack of comprehensive analysis. In this paper, we propose BiasPainter, a novel evaluation framework that can accurately, automatically and comprehensively trigger social bias in image generation models. BiasPainter uses a diverse range of seed images of individuals and prompts the image generation models to edit these images using gender, race, and age-neutral queries. These queries span 62 professions, 39 activities, 57 types of objects, and 70 personality traits. The framework then compares the edited images to the original seed images, focusing on the significant changes related to gender, race, and age. BiasPainter adopts a key insight that these characteristics should not be modified when subjected to neutral prompts. Built upon this design, BiasPainter can trigger the social bias and evaluate the fairness of image generation models. We use BiasPainter to evaluate six widely-used image generation models, such as stable diffusion and Midjourney. Experimental results show that BiasPainter can successfully trigger social bias in image generation models. According to our human evaluation, BiasPainter can achieve 90.8% accuracy on automatic bias detection, which is significantly higher than the results reported in previous work.

==> Sections/5_Discussion.tex <==
\section{Threats to Validity}
\label{sec-discuss}


The validity of this work may be subject to some threats.
The first threat lies in the AI techniques adopted by \methodname for bias identification. 
Due to the imperfect nature of AI techniques, the biases identified by \methodname may be false positives, or \methodname may miss some biased generation, leading to false negatives.
To relieve this threat, \methodname calls commercial-level APIs and deploys complicated pipelines to analyze the race, gender, and age properties, aiming to ensure soundness.
In addition, we also conducted human annotation to show that \methodname can achieve high accuracy (\ie 90.8\%) in detecting bias.

The second threat is that the input data of \methodname are predefined, both seed images and prompt lists, which may hurt the comprehensiveness of the testing results. 
To mitigate this threat, we collected diverse and comprehensive seed images and prompt words, all of which are from the real world on the Internet and manually annotated by researchers. 
Also, we want to highlight that what we provide is a workflow: select seed images, design prompt lists, generate test cases, and find social bias.
If users are willing to evaluate other properties on other images, they could follow this workflow to add more images and prompts.

\iffalse
The third threat lies in the image generation models under test in the evaluation. We do not evaluate the performance of \methodname on other systems.
To mitigate this threat, we chose to test the most widely used commercial image generation software and SOTA academic models provided by famous organizations.
In the future, we could test more commercial software and research models to further mitigate this threat.
\fi
